A practical fpt algorithm for Flow Decomposition and transcript assembly

The Flow Decomposition problem, which asks for the smallest set of weighted paths that "covers" a flow on a DAG, has recently been used as an important computational step in transcript assembly. We prove the problem is in FPT when parameterized by the number of paths by giving a practical linear fpt algorithm. Further, we implement and engineer a Flow Decomposition solver based on this algorithm, and evaluate its performance on RNA-sequence data. Crucially, our solver finds exact solutions while achieving runtimes competitive with a state-of-the-art heuristic. Finally, we contextualize our design choices with two hardness results related to preprocessing and weight recovery. Specifically, $k$-Flow Decomposition does not admit polynomial kernels under standard complexity assumptions, and the related problem of assigning (known) weights to a given set of paths is NP-hard.

==> figures/table_entry.tex <==
\begin{tikzpicture}
	\tikzset{vertex/.style = {shape=circle,fill=white,draw,minimum size=0.75cm}}
	\tikzset{arc/.style = {->, line width=1pt}}
	\tikzset{flowlabel/.style = {sloped,anchor=south}}

	\node[rectangle,
	      draw,
	      minimum height=8cm,
	      minimum width=1.5cm,
	      fill=blue!50,
	      label=above:{$S_i$}] (Si) at (0,3) {};

	\node[rectangle,
	      draw,
	      minimum height=6cm,
	      minimum width=1.5cm,
	      fill=red!50,
	      label=above:{$N^+(S_i)$}] (Ni) at (6,3) {};

	\node[ellipse,
	      draw,
	      minimum height=7cm,
	      minimum width=2.0cm,
	      fill=black!30,
	      label=above:{$g$}] (g) at (3,3) {};

	\node[vertex] (v4) at (0,0) {$v_4$};
	\node[vertex] (v3) at (0,2) {$v_3$};
	\node[vertex] (v2) at (0,4) {$v_2$};
	\node[vertex] (v1) at (0,6) {$v_1$};

	\node[vertex] (u3) at (6,1) {$u_3$};
	\node[vertex] (u2) at (6,3) {$u_2$};
	\node[vertex] (u1) at (6,5) {$u_1$};


	\draw[arc] (v1) edge node [flowlabel] {$1, 4$}    (u1);
	\draw[arc] (v1) edge node [flowlabel] {$3, 5, 6$} (u2);
	\draw[arc] (v2) edge node [flowlabel] {$2$}       (u2);
	\draw[arc] (v4) edge node [flowlabel] {$7$}       (u3);
	\draw[arc] (v3) edge node [flowlabel] {$8$}       (u2);

	% \node[label=above:{$L_g$}] (table) at (11,3) {
	% $\left[
	% \begin{array}{c c c c c c c c |c}
	% 	1 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & f(v_1u_1)\\
	% 	0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & f(v_2u_2)\\
	% 	0 & 0 & 1 & 0 & 1 & 1 & 0 & 0 & f(v_1u_2)\\
	% 	0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & f(v_4u_3)\\
	% 	0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & f(v_3u_2)\\
	% \end{array}\right]$
	% };

\end{tikzpicture}


==> figures/table_entry_matrix.tex <==
\begin{tikzpicture}

\node[label=above:{$L_g$}] (table) at (1,1) {
$\left[
\begin{array}{c c c c c c c c |c}
  1 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & f(v_1u_1)\\
  0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & f(v_2u_2)\\
  0 & 0 & 1 & 0 & 1 & 1 & 0 & 0 & f(v_1u_2)\\
  0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & f(v_4u_3)\\
  0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & f(v_3u_2)\\
\end{array}\right]$
};


\end{tikzpicture}


==> figures/topological-ordering.tex <==
\begin{tikzpicture}


\tikzset{vertex/.style = {shape=circle,draw,minimum size=0.75cm}}
\tikzset{arc/.style = {->, line width=1pt}}


%%%
%%% DRAW NODES
%%%
\node[vertex] (s) at (0,0) {$v_1$};
\node[vertex] (2) at (2.5,0){$v_2$};
\node[vertex] (3) at (5,0){$v_3$};
\node (d) at (7.5,0){$\cdots$};
\node[vertex] (t) at (10,0){$v_n$};


%%%
%%% DRAW BOX
%%%
\draw[black,thick,dashed] (-0.75,-0.75) rectangle (5.75,1) node[label=$S_3$, at start, pos=-0.075] {};


%%%
%%%  DRAW ARCS
%%%
\draw[arc] (s)  to  (2);
\draw[arc] (s)  to[bend left] (3);
\draw[arc] (2)  to (3);
\draw[arc] (s)  to[bend left=45] (d);
\draw[arc] (3)  to[bend right] (d);
\draw[arc] (d)  to[bend left] (t);

\end{tikzpicture}


==> figures/x3h-reduction.tex <==
\begin{tikzpicture}

\def \thinlinewidth {1pt}
\def \mediumlinewidth {2pt}
\def \thicklinewidth {3pt}

\def \innerlooseness {0.6}
\def \outerlooseness {1.3}
\def \greencolor {black!45!green}


\tikzset{vertex/.style = {shape=circle,draw,minimum size=0.65cm}}
\tikzset{arc/.style = {->, line width=1pt}}

\node[vertex] (s) at (0,0){\small{s}};
\node[vertex] (1) at (1.75,0){\small{1}};
\node[vertex] (2) at (3.5,0){\small{2}};
\node[vertex] (3) at (5.25,0){\small{3}};
\node[vertex] (4) at (7,0){\small{4}};
\node[vertex] (t) at (8.75,0){\small{t}};


%%
%% NODE s TO 1
%%
% \draw[arc] (s)  to["\tiny{$A\bar{A}, 3$}", out=90, in=90, looseness=1.4] (1);
% \draw[arc] (s)  to["\tiny{$B\bar{B}, 3$}", out=55, in=125, looseness=0.8] (1);
% \draw[arc] (s)  to["\tiny{$C\bar{C}, 3$}"] (1);
% \draw[arc] (s)  to["\tiny{$D\bar{D}, 3$}", out=305, in=235, looseness=0.8] (1);
% \draw[arc] (s)  to["\tiny{$E\bar{E}, 3$}", out=270, in=270, looseness=1.4] (1);
\draw[arc] (s)  to[out=90, in=90, looseness=1.4] node[midway, above] {\tiny{$A\bar{A}, 3$}} (1) ;
\draw[arc] (s)  to[out=55, in=125, looseness=0.8] node[midway, above] {\tiny{$B\bar{B}, 3$}} (1) ;
\draw[arc] (s)  to node[midway, above] {\tiny{$C\bar{C}, 3$}} (1);
\draw[arc] (s)  to[out=305, in=235, looseness=0.8] node[midway, above] {\tiny{$D\bar{D}, 3$}} (1);
\draw[arc] (s)  to[out=270, in=270, looseness=1.4] node[midway, above] {\tiny{$E\bar{E}, 3$}} (1);

%%
%%  NODE 1 TO 2
%%
% \draw[arc] (1)  to["\tiny{$D\bar{D}, 3$}", out=80, in=100, looseness=\outerlooseness] (2);
% \draw[arc] (1)  to["\tiny{$E\bar{E}, 3$}", out=45, in=135, looseness=\innerlooseness] (2);
% \draw[arc, line width=\mediumlinewidth] (1)  to["\tiny{$ABC, 4$}", out=315, in=225, looseness=\innerlooseness] (2);
% \draw[arc, line width=\thicklinewidth] (1)  to["\tiny{$\bar{A}\bar{B}\bar{C}, 5$}", out=280, in=260, looseness=\outerlooseness] (2);
\draw[arc] (1)  to[out=80, in=100, looseness=\outerlooseness] node[midway, above] {\tiny{$D\bar{D}, 3$}} (2);
\draw[arc] (1)  to[out=45, in=135, looseness=\innerlooseness] node[midway, above] {\tiny{$E\bar{E}, 3$}} (2);
\draw[arc, line width=\mediumlinewidth] (1)  to[out=315, in=225, looseness=\innerlooseness] node[midway, above] {\tiny{$ABC, 4$}} (2);
\draw[arc, line width=\thicklinewidth] (1)  to[out=280, in=260, looseness=\outerlooseness] node[midway, above] {\tiny{$\bar{A}\bar{B}\bar{C}, 5$}} (2);

%%
%%  NODE 2 TO 3
%%
% \draw[arc] (2)  to["\tiny{$C\bar{C}, 3$}", out=80, in=100, looseness=\outerlooseness] (3);
% \draw[arc] (2)  to["\tiny{$E\bar{E}, 3$}", out=45, in=135, looseness=\innerlooseness] (3);
% \draw[arc, line width=\mediumlinewidth] (2)  to["\tiny{$ABD, 4$}", out=315, in=225, looseness=\innerlooseness] (3);
% \draw[arc, line width=\thicklinewidth] (2)  to["\tiny{$\bar{A}\bar{B}\bar{D}, 5$}", out=280, in=260, looseness=\outerlooseness] (3);
\draw[arc] (2)  to[out=80, in=100, looseness=\outerlooseness] node[midway, above] {\tiny{$C\bar{C}, 3$}} (3);
\draw[arc] (2)  to[out=45, in=135, looseness=\innerlooseness] node[midway, above] {\tiny{$E\bar{E}, 3$}} (3);
\draw[arc, line width=\mediumlinewidth] (2)  to[out=315, in=225, looseness=\innerlooseness] node[midway, above, color = red] {\tiny{$ABD, 4$}} (3);
\draw[arc, line width=\thicklinewidth] (2)  to[out=280, in=260, looseness=\outerlooseness] node[midway, above] {\tiny{$\bar{A}\bar{B}\bar{D}, 5$}} (3);

%%
%%  NODE 3 TO 4
%%
% \draw[arc] (3)  to["\tiny{$A\bar{A}, 3$}", out=80, in=100, looseness=\outerlooseness] (4);
% \draw[arc] (3)  to["\tiny{$D\bar{D}, 3$}", out=45, in=135, looseness=\innerlooseness] (4);
% \draw[arc, line width=\mediumlinewidth] (3)  to["\tiny{$BCE, 4$}", out=315, in=225, looseness=\innerlooseness] (4);
% \draw[arc, line width=\thicklinewidth] (3)  to["\tiny{$\bar{B}\bar{C}\bar{E}, 5$}", out=280, in=260, looseness=\outerlooseness] (4);
\draw[arc] (3)  to[out=80, in=100, looseness=\outerlooseness] node[midway, above] {\tiny{$A\bar{A}, 3$}} (4);
\draw[arc] (3)  to[out=45, in=135, looseness=\innerlooseness] node[midway, above] {\tiny{$D\bar{D}, 3$}} (4);
\draw[arc, line width=\mediumlinewidth] (3)  to[out=315, in=225, looseness=\innerlooseness] node[midway, above, color = blue] {\tiny{$BCE, 4$}} (4);
\draw[arc, line width=\thicklinewidth] (3)  to[out=280, in=260, looseness=\outerlooseness] node[midway, above] {\tiny{$\bar{B}\bar{C}\bar{E}, 5$}} (4);

%node[midway, above] {}
%%
%%  NODE 3 TO 4
%%
% \draw[arc] (4)  to["\tiny{$A\bar{A}, 3$}", out=80, in=100, looseness=\outerlooseness] (t);
% \draw[arc] (4)  to["\tiny{$B\bar{B}, 3$}", out=45, in=135, looseness=\innerlooseness] (t);
% \draw[arc, line width=\mediumlinewidth] (4)  to["\tiny{$CDE, 4$}", out=315, in=225, looseness=\innerlooseness] (t);
% \draw[arc, line width=\thicklinewidth] (4)  to["\tiny{$\bar{C}\bar{D}\bar{E}, 5$}", out=280, in=260, looseness=\outerlooseness] (t);
\draw[arc] (4)  to[out=80, in=100, looseness=\outerlooseness] node[midway, above] {\tiny{$A\bar{A}, 3$}} (t);
\draw[arc] (4)  to[out=45, in=135, looseness=\innerlooseness] node[midway, above] {\tiny{$B\bar{B}, 3$}} (t);
\draw[arc, line width=\mediumlinewidth] (4)  to[out=315, in=225, looseness=\innerlooseness] node[midway, above, color = \greencolor] {\tiny{$CDE, 4$}} (t);
\draw[arc, line width=\thicklinewidth] (4)  to[out=280, in=260, looseness=\outerlooseness] node[midway, above] {\tiny{$\bar{C}\bar{D}\bar{E}, 5$}} (t);

\end{tikzpicture}


==> macros-preamble.tex <==


